Let Me Speak Freely? A Study on the Impact of Format Restrictions on Performance of Large Language Models

Structured generation, the process of producing content in standardized formats like JSON and XML, is widely utilized in real-world applications to extract key output information from large language models (LLMs). This study investigates whether such constraints on generation space impact LLMs abilities, including reasoning and domain knowledge comprehension. Specifically, we evaluate LLMs performance when restricted to adhere to structured formats versus generating free-form responses across various common tasks. Surprisingly, we observe a significant decline in LLMs reasoning abilities under format restrictions. Furthermore, we find that stricter format constraints generally lead to greater performance degradation in reasoning tasks.

==> figs/showcase_fig.tex <==
\begin{figure}[htbp]
\centering
\begin{minipage}{0.95\textwidth}
\begin{tcolorbox}[title=Standard Prompting]
%prompt here

\rule{\linewidth}{0.4pt}

Instruct : Provide your output in the following text format:\\
Step by step reasoning: ... \\
Answer: The final answer is ...\\
\textbf{\# Response}\\
Step by step reasoning: \\
1. Eliza's regular rate per hour is \$10 for the first 40 hours.\\
2. For the 5 hours of overtime, her rate is 1.2 times her regular rate, which is 1.2 * \$10 = \$12 per hour.\\
3. Eliza worked 40 regular hours and 5 overtime hours, totaling 45 hours.\\
4. Earnings for regular hours = 40 hours * \$10/hour = \$400\\
5. Earnings for overtime hours = 5 hours * \$12/hour = \$60\\
6. Total earnings for the week = \$400 (regular) + \$60 (overtime) = \$460\\

Answer: The final answer is 460.

\end{tcolorbox}

\vspace{1em}

\begin{tcolorbox}[title=Format-Restricting Prompting]

Instruct : Provide your output in the following \\valid JSON format:\\
```json\\
\{\\
    "step\_by\_step\_reasoning": ...,\\
    "answer": ...\\
\}\\
```\\

\rule{\linewidth}{0.4pt}

\textbf{\# Responses to a batch}
```json\\
\{
    "step\_by\_step\_reasoning": "Calculate the earnings for the first 40 hours at \$10 per hour. Then calculate the earnings for the additional 5 hours at \$10 * 1.2 per hour. Add both amounts to find the total earnings for the week.",\\
    "answer": 490\\
\}
```\\

\end{tcolorbox}
\end{minipage}
\caption{Comparison of Standard and Batch Prompting}
\label{fig:prompting_comparison}
\end{figure}
